Browser Fingerprinting: A survey

With this paper, we survey the research performed in the domain of browser fingerprinting, while providing an accessible entry point to newcomers in the field. We explain how this technique works and where it stems from. We analyze the related work in detail to understand the composition of modern fingerprints and see how this technique is currently used online. We systematize existing defense solutions into different categories and detail the current challenges yet to overcome.

==> parts/4-usage.tex <==
\section{Usage of browser fingerprinting}
\label{sec:usage}

Building a browser fingerprint can give many details on a device and its configuration.
The use of the collected information falls into two main categories.

\begin{itemize}
\item \textbf{Negative or destructive use} An unknown third party would want to track a user without her consent or to attack her device by identifying a known vulnerability.
\item \textbf{Positive or constructive use} Users can be warned if their device is out of date by recommending specific updates.
The security of online services can also be reinforced by verifying that a device is genuine and that it is known to the system. 
\end{itemize}


\subsection{Tracking}
\label{subsec:tracking}

As browser fingerprinting can uniquely identify a device on the web, the implications on privacy are important.
By collecting browser fingerprints on several websites, a third party can recognize a user and correlate his browsing activity within and across sessions.
Most importantly, the user has no control over the collection process as it is completely transparent since the tracking scripts are silent and executed in the background.
The Panopticlick study outlines in more details how fingerprinting can a be a threat to web privacy~\cite{eckersley2010Pano}.

\begin{itemize}
\item \textbf{Fingerprints as Global Identifiers} If a device has a fingerprint that is unique, it can be identified on the web without the need of other identifiers like a cookie or an IP address.
Peter Eckersley add in his study that it is ``akin to a cookie that cannot be deleted''.
Users funneling their network packets through a VPN (Virtual Private Network) are particularly vulnerable to browser fingerprinting as the VPN will only mask the IP address but it will not change the browser's information.

\item \textbf{Fingerprint + IP address as Cookie Regenerators}
Coupled with a fixed IP address, a browser fingerprint can be used to regenerate deleted cookies.
Researchers have already observed in the wild that any browser storage mechanisms like Flash local storage~\cite{soltani2010flash}, HTML5 Web storage~\cite{ayenson2011flash} or IndexedDB databases~\cite{acar14neverForgets}, can be used to ``respawn'' HTTP cookies.

\item \textbf{Fingerprint + IP address in the Absence of Cookies} In the absence of cookies, browser fingerprinting can be used to unmask different machines hiding behind the same IP address.
\end{itemize}

\subsection{Identifying device vulnerabilities}
\label{subsec:vulnerabilities}
A browser fingerprint is not just a simple collection of device-specific information.
It truly reflects the actual set of components that are running on a device.
By analysing its content, attackers can identify potential security vulnerabilities by cross-referencing the list of installed components with a database like CVE (Common Vulnerabilities and Exposures~\cite{cveWebsite}).
They can then design the perfect payload to target a specific device knowing its vulnerabilities in advance.
For example, through the \textit{navigator.plugins} property, one can know if a device is running an outdated version of the Flash plugin.
At the time of writing, the CVE database reports 1,045 Flash vulnerabilities and more than 84\% are labelled as critical, including the most recent ones~\cite{cveFlash}.
If the Flash player is not up to date, users open themselves to serious security risks as any attacker on the web could execute malicious code remotely on their device.

Launching a targeted attack with the help of browser fingerprinting is not new and has been observed in the wild.
Malwarebytes and GeoEdge have documented extensively with the ``Operation fingerprint'' how malicious advertising campaigns use fingerprinting to deliver malwares to vulnerable devices~\cite{operatinFingerprint}.
Their process is very straightforward.
They hide fingerprinting code directly into the JavaScript of fake advertisers and they look from there if the device is vulnerable or not.
If it is, the device will be presented with ``an ad laced with malicious code that ultimately redirects to an exploit kit''.
If it is not, the ad will be ``benign''.
To illustrate their findings, they detail several types of malvertising campaigns like the \textit{DoubleClick} or the \textit{musical4} campaigns.


\subsection{Improving security on the web}
\label{subsec:security}

\subsubsection{Patching vulnerable systems}
Directly following the previous section, browser vulnerabilities could be identified with the aim of patching them.
In 2015, Duo Security reported that 46\% of corporate PCs ran outdated versions of browsers, Flash and Java~\cite{duoVulnerabilities}.
With a simple security scan, system administrators who handle thousands of different configurations on a network could easily identify devices with outdated components and they could deploy fixes and updates really quickly.

\subsubsection{Bot and fraud prevention}
Another use of browser fingerprinting is to improve security on the web by verifying the actual content of a fingerprint.
As there are many dependencies between collected attributes, it is possible to check if a fingerprint has been tampered with or if it matches the device it is supposedly belonging to (see Section~\ref{subsec:increasing} for details on the inconsistency problem).

ThreatMetrix, a security company that specializes in the verification of online transactions, announced in 2010 the adoption of browser fingerprinting techniques to prevent online fraud~\cite{FPthreatmetrix}.
They wrote that fraudsters change their IP address, delete cookies and botnet scripts randomize device attributes.
Moreover, relying exclusively on cookies is no longer adequate to verify an online transaction.
Other security companies like Distil Networks~\cite{FPdistil}, MaxMind~\cite{FPmaxmind}, PerimeterX~\cite{FPPermiter}, IPQualityScore~\cite{FPQuality}, ShieldSquare~\cite{FPShieldSquare} or Sift Science~\cite{FPSift} also utilize browser fingerprinting to detect bots and unusual activity.
In that landscape, companies are turning to browser fingerprinting to be competitive in this continual arms race against fraudsters.

On the academic side, the literature on fraud detection is much thinner with only a single publication addressing this problem.
Researchers at Google designed a solution called Picasso based on canvas fingerprinting to filter inorganic traffic~\cite{bursztein2016Picasso}.
By using specific graphical primitives from the canvas API, they are able to successfully detect the browser and OS family of a device and see if there is a mismatch between the exhibited fingerprint and the actual device running the code.
For example, they can distinguish between traffic sent by an authentic iPhone running Safari on iOS from an emulator or desktop client spoofing the same configuration.
They add that the applications are numerous including locking non-mobile clients from application marketplaces, detecting rogue login attempts and identifying emulated clients.
Their study does not give information on the deployment of Picasso in a current Google solution but a talk at Black Hat Asia 2016 hints at its integration into Google's reCAPTCHA technology~\cite{sivakornm16recaptcha}.

\subsubsection{Augmented authentication}
At a time where passwords are the go-to solution for authentication on the web, browser fingerprinting can provide a much needed addition to reinforce the security of online accounts.
By verifying the fingerprint of a device at login time, a system can easily block unauthorized access from new and unknown devices.
Alaca et al. studied extensively the use of device fingerprinting for web authentication~\cite{alaca2016Authentication}. 
They classify in total 29 different attributes from browser information to the network stack according to criteria like repeatability, low resource use or spoofing resistance.
One important aspect considered in their study is the notion of stability.
As a fingerprint is the direct reflection of what is installed on a device, a browser fingerprint constantly changes. 
It is then up to the login system to decide if the differences between two fingerprints are acceptable or not.
For example, does a change of browser version in the user-agent come from a legitimate update of the device or from a different device altogether?
If ten fonts are removed, did the user uninstall a particular software or does it come from a different device that does not belong to the user?
These questions have no easy answer and each collected attribute has its own behavior depending on the system being used or the type of the device.
Spooren et al. looked at mobile devices and noticed that mobile fingerprints are predictable contrarily to desktop fingerprints~\cite{spooren2015MobileFPHarmful}.
The same authors also investigated the use of battery information for mobile devices in a multi-factor authentication scheme~\cite{spoorenPJ17}.
By using binary classifiers to classify battery draining and charging behaviors, they confirm that battery charge measurements can be used to contribute to an active authentication system.

Finally, some companies include in their portfolio fingerprinting solutions to augment authentication.
SecurAuth is a provider of an adaptive access control solution. 
As part of their multi-factor authentication process, they include an heuristic-based authentication system through device fingerprinting~\cite{securauth}.
Another company called Iovation has a solution named ClearKey~\cite{clearkey} that integrates the collection of device information as part of their multi-factor authentication framework.
They provide their own approach to deal with fingerprint changes with fuzzy logic algorithms~\cite{clearkeySheet}.

All in all, the amount of research done to use browser fingerprinting positively is extremely thin and we hope that this area will see major advancements in the future.

==> parts/8-appendices.tex <==
\appendix

\section{Complementary tables}
\label{appendices}


%\newcommand{\comments}{8.0cm}
%\newcommand{\plusminus}[2]{\parbox[c]{\comments}{\vspace{.3\baselineskip} $+$: #1\\$-$: #2 \vspace{.3\baselineskip}} }

\begin{table*}[h!]
\caption{Summary of existing defense solutions.
M = Modifying the fingerprint content. 
M* = Modifying the fingerprint content by switching browsers.
U = Universal fingerprint.
BS = Blocking Scripts.
BA = Blocking APIs.
}
\center
\scalebox{0.99}{
%\begin{tabular}{|*5{c|}}
\begin{tabular}{M{0.001cm} | M{3cm} | M{2cm} | M{2cm} | M{\comments} }
%     \cline{2-5}
     \multicolumn{1}{c|}{\multirow{1}{*}{}} & Solution & Ref. & Type & Comments\\\hline
     \multirow{20}{*}{\rotatebox[origin=c]{90}{Scientific publications}} & FP-Block & \cite{torres15FPBlock} & M 
	 & \plusminus{Separation of web identities}{Incomplete coverage} \\\cline{2-5}
     & FPGuard & \cite{faiz15FPguard} & M 
     & \plusminus{Detection and prevention of fingerprinting}{Lack of details} \\\cline{2-5}
     & Fiore et al. & \cite{fiore14countering} & M 
     & \plusminus{Aims at creating consistent fingerprints}{Incomplete coverage} \\\cline{2-5}
     & DCB & \cite{baumann16disguised} & M 
     & \plusminus{N:1/1:N strategies, changes at each session, creation of groups with similar configurations}{Incomplete coverage}  \\\cline{2-5}
     & PriVaricator & \cite{nikiforakis15Privari} & M 
     & \plusminus{Custom randomization policies}{Incomplete coverage} \\\cline{2-5}
     & Blink & \cite{laperdrix15Mitigating} & M 
     & \plusminus{Produces genuine and diverse fingerprints with no inconsistencies}{Takes HDD space} \\\cline{2-5}
	 & FPRandom & \cite{laperdrix17fprandom} & M 
	 & \plusminus{Introduces noise into the Canvas, AudioContext APIs and randomizes the enumeration order of JavaScript objects}{Other vectors can still be used} \\\cline{2-5}
     & Changing browsers & \cite{boda12crossBrowser,cao17cross} & M* 
     & \plusminus{Presents distinct and genuine fingerprints}{Can be bypassed} \\\cline{2-5}
     & Cliqz browser & \cite{yu16cliqz,cliqz} & BS 
     & \plusminus{Strong protection against scripts with unique identifiers}{Relies on a central server} \\\cline{2-5}\hline
          
	 \multirow{23}{*}{\rotatebox[origin=c]{90}{Online tools}} & Canvas Defender & \cite{canvasDefender} & M 
	 & \plusminus{Modifications consistent across a browsing session}{Only canvas} \\\cline{2-5}
     & Random Agent Spoofer & \cite{randomSpoofer} & M 
     & \plusminus{Uses real database of browser profiles}{Incomplete coverage} \\\cline{2-5}
     & Tor Browser & \cite{torBrowser} & U BA 
     & \plusminus{Very strong protection against fingerprinting }{Tor fingerprint is brittle} \\\cline{2-5}
     & NoScript & \cite{noscript} & BS 
     & \plusminus{Blocks all JavaScript scripts including fingerprinting scripts}{Blocks all JavaScript scripts including scripts needed to correctly display a webpage} \\\cline{2-5}
     & Adblock Plus & \cite{adblockplus} & BS 
     & \plusminus{Extensive blocking list}{Relies on lists of known trackers} \\\cline{2-5}
     & Ghostery & \cite{ghostery} & BS 
     & \plusminus{Very extensive blocking list}{Relies on lists of known trackers} \\\cline{2-5}
     & uBlock Origin & \cite{ublockGithub} & BS 
     & \plusminus{Extensive blocking list}{Relies on lists of known trackers} \\\cline{2-5}
     & Disconnect & \cite{disconnect} & BS 
     & \plusminus{Very extensive blocking list}{Relies on lists of known trackers} \\\cline{2-5}
     & Privacy Badger & \cite{privacyBadger} & BS 
     & \plusminus{Heuristics-based approach}{Blocking may be too aggressive} \\\cline{2-5}
	 & Canvas Blocker & \cite{canvasBlocker} & BA 
	 & \plusminus{Blocks the entire canvas API}{Other vectors can still be used} \\\cline{2-5}
	 & Brave browser & \cite{brave} & BA 
	 & \plusminus{Blocks the entire Canvas, WebGL, AudioContext and WebRTC APIs}{Other vectors can still be used} \\\cline{2-5}
	 & Firefox fingerprinting resistance & \cite{firefoxProtection,torUplift,firefoxFusion} & M BA U& \plusminus{Blocks the entire Canvas API and reduces the quantity of information on several attributes}{Still a work in progress, other vectors can still be used} \\
	 %\cline{2-5}\hline
\end{tabular}
}

\label{background:table:defenses}
\end{table*}

